Parity Polytopes and Binarization

We consider generalizations of parity polytopes whose variables, in addition to a parity constraint, satisfy certain ordering constraints. More precisely, the variable domain is partitioned into $k$ contiguous groups, and within each group, we require that $x_i \geq x_{i+1}$ for all relevant $i$. Such constraints are used to break symmetry after replacing an integer variable by a sum of binary variables, so-called binarization. We provide extended formulations for such polytopes, derive a complete outer description, and present a separation algorithm for the new constraints. It turns out that applying binarization and only enforcing parity constraints on the new variables is often a bad idea. For our application, an integer programming model for the graphic traveling salesman problem, we observe that parity constraints do not improve the dual bounds, and we provide a theoretical explanation of this effect.

==> tikz-extended-formulations-ordered-parity.tex <==
\piDeclareString{job}{}
\piDeclareBool{debug}{false}

\piParse % Parses all given options

\piIfString{job}{config}{%
  % Preamble code
  \usetikzlibrary{shapes.geometric}
}{

% Debugging code

\piIfString{job}{network}{

\def\boundingbox{(-0.25,-0.25) rectangle (10.25,2.25)};
\draw[clip,use as bounding box,draw=none] \boundingbox;
\piIfBool{debug}{
  \draw[step=.5cm,help lines] (-11,-20) grid (11,20);
  \draw[draw=red,thick] \boundingbox;
}{}

\foreach \name/\x/\y in {s/0/0, a/1.5/0, b/1.5/1, c/3/0, d/3/1, e/4.5/0, f/4.5/1, g/7/0, h/7/1, i/8.5/0, j/8.5/1, t/10/0} {
  \node[draw=black,fill=black!20!white,circle, minimum size=3mm, inner sep=0mm] (\name) at (\x,2-1.5*\y) {};
}

\foreach \from/\to in {s/a, s/b, a/c, a/d, b/c, b/d, c/e, c/f, d/e, d/f, g/i, g/j, h/i, h/j, i/t, j/t} {
  \draw[very thick,->] (\from) -- (\to);
}

\node at (5.75,2-0.75) {{\Huge{$\ldots$}}};
\node at (0,1.6) {$s$};
\node at (10,1.6) {$t$};

\foreach \x/\i in {0/1, 1.5/2, 3/3, 7/{n-1}, 8.5/{n}} {
  \node at (\x+0.75,0.0) {\footnotesize{$i=\i$}};
}

}{} % job == network

\piIfString{job}{default-level}{
  \def\boundingbox{(-0.25,-0.25) rectangle (10.25,3.25)};
  \draw[clip,use as bounding box,draw=none] \boundingbox;
  \piIfBool{debug}{
    \draw[step=.5cm,help lines] (-11,-20) grid (11,20);
    \draw[draw=red,thick] \boundingbox;
  }{}
  
  \def\shift{1}

  \draw[black,fill=black!20!white] (\shift+1,2.5) ellipse (0.7 and 0.6);
  \draw[black,fill=black!20!white] (\shift+1,0.5) ellipse (0.7 and 0.6);
  \draw[black,fill=black!20!white] (\shift+4,2.5) ellipse (0.7 and 0.6);
  \draw[black,fill=black!20!white] (\shift+4,0.5) ellipse (0.7 and 0.6);
  
  \node (a) at (\shift+1,2.5) {$(i-1,0)$};
  \node (b) at (\shift+1,0.5) {$(i-1,1)$};
  \node (c) at (\shift+4,2.5) {$(i,0)$};
  \node (d) at (\shift+4,0.5) {$(i,1)$};
  
  \draw[very thick,->] (\shift+1.7,0.5) -- (\shift+3.3,0.5);
  \draw[very thick,->] (\shift+1.7,2.5) -- (\shift+3.3,2.5);
  \draw[decorate,decoration={zigzag,amplitude=0.4mm,segment length=2mm,pre length=1mm, post length=1mm},very thick,->] (\shift+1.6,0.8) -- (\shift+3.4,2.2);
  \draw[decorate,decoration={zigzag,amplitude=0.4mm,segment length=2mm,pre length=1mm, post length=1mm},very thick,->] (\shift+1.6,2.2) -- (\shift+3.4,0.8);
  
  \node[anchor=west] at (0,1.5) {$r_i = 1$:};
  \node[anchor=west] at (\shift+5,1.5) {$x^{(i)}_1 = \sum y_{\left(\begin{tikzpicture}\draw[decorate,decoration={zigzag,amplitude=0.4mm,segment length=1mm},thick] (0,0) -- (0.4,0);\end{tikzpicture}\right)}$};
}{} % job == default-level


\piIfString{job}{ordered-level}{
  \def\boundingbox{(-0.25,-0.25) rectangle (10.25,3.25)};
  \draw[clip,use as bounding box,draw=none] \boundingbox;
  \piIfBool{debug}{
    \draw[step=.5cm,help lines] (-11,-20) grid (11,20);
    \draw[draw=red,thick] \boundingbox;
  }{}
  
  \def\shift{1}

  \draw[black,fill=black!20!white] (\shift+1,2.5) ellipse (0.7 and 0.6);
  \draw[black,fill=black!20!white] (\shift+1,0.5) ellipse (0.7 and 0.6);
  \draw[black,fill=black!20!white] (\shift+4,2.5) ellipse (0.7 and 0.6);
  \draw[black,fill=black!20!white] (\shift+4,0.5) ellipse (0.7 and 0.6);
  
  \node (a) at (\shift+1,2.5) {$(i-1,0)$};
  \node (b) at (\shift+1,0.5) {$(i-1,1)$};
  \node (c) at (\shift+4,2.5) {$(i,0)$};
  \node (d) at (\shift+4,0.5) {$(i,1)$};
  
  \draw[very thick,->] (\shift+1.7,0.5) to[bend left=10)] (\shift+3.3,0.5);
  \draw[very thick,->] (\shift+1.7,2.5) to[bend right=10] (\shift+3.3,2.5);
  \draw[decorate,decoration={triangles,segment length=1.35mm},thick,->] (\shift+1.7,0.3) to[bend right=10] (\shift+3.3,0.3);
  \draw[decorate,decoration={triangles,segment length=1.35mm},thick,->] (\shift+1.7,2.7) to[bend left=10] (\shift+3.3,2.7);
  \draw[decorate,decoration={zigzag,amplitude=0.4mm,segment length=2mm,pre length=1mm, post length=1mm},very thick,->] (\shift+1.6,0.8) to[bend right=20] (\shift+3.5,2.1);
  \draw[decorate,decoration={zigzag,amplitude=0.4mm,segment length=2mm,pre length=1mm, post length=1mm},very thick,->] (\shift+1.6,2.2) to[bend left=20] (\shift+3.5,0.9);
  \draw[dashed,very thick,->] (\shift+1.6,0.8) to[bend left=15] (\shift+3.4,2.2);
  \draw[dashed,very thick,->] (\shift+1.6,2.2) to[bend right=15] (\shift+3.4,0.8);
  
  \node[anchor=west] at (0,1.5) {$r_i = 3$:};
  \node[anchor=west] at (\shift+5,2.4) {$x^{(i)}_3 = 
    \sum y_{(\begin{tikzpicture}\draw[dashed,very thick] (0,0) -- (0.35,0);\end{tikzpicture})}
  $};
  \node[anchor=west] at (\shift+5,1.5) {$x^{(i)}_2 = 
    \sum y_{\left(\begin{tikzpicture}\draw[decorate,decoration={triangles,segment length=1.4mm},thick] (0,0) -- (0.4,0);\end{tikzpicture}\right)}
    + x^{(i)}_3$};
  \node[anchor=west] at (\shift+5,0.6) {$x^{(i)}_1 = 
    \sum y_{\left(\begin{tikzpicture}\draw[decorate,decoration={zigzag,amplitude=0.4mm,segment length=1mm},thick] (0,0) -- (0.4,0);\end{tikzpicture}\right)}
    + x^{(i)}_2$};
}{} % job == ordered-level

} % job == config

